Formulating and solving integrated order batching and routing in multi-depot AGV-assisted mixed-shelves warehouses

Different retail and e-commerce companies are facing the challenge of assembling large numbers of time-critical picking orders that include both small-line and multi-line orders. To reduce unproductive picker working time as in traditional picker-to-parts warehousing systems, different solutions are proposed in the literature and in practice. For example, in a mixed-shelves storage policy, items of the same stock keeping unit are spread over several shelves in a warehouse; or automated guided vehicles (AGVs) are used to transport the picked items from the storage area to packing stations instead of human pickers. This is the first paper to combine both solutions, creating what we call AGV-assisted mixed-shelves picking systems. We model the new integrated order batching and routing problem in such systems as an extended multi-depot vehicle routing problem with both three-index and two-commodity network flow formulations. Due to the complexity of the integrated problem, we develop a novel variable neighborhood search algorithm to solve the integrated problem more efficiently. We test our methods with different sizes of instances, and conclude that the mixed-shelves storage policy is more suitable than the usual storage policy in AGV-assisted mixed-shelves systems for orders with different sizes of order lines (saving up to 62% on driving distances for AGVs). Our variable neighborhood search algorithm provides optimal solutions within an acceptable computational time.

==> bib.tex <==
% Encoding: UTF-8
﻿% This file was created with Citavi 5.5.0.1

@book{.,
 title = {9th International Quality Conference 2015}
}


@book{.1996,
 year = {1996},
 title = {Proceedings of the Twelfth international conference on Uncertainty in artificial intelligence},
 address = {Portland, OR},
 publisher = {{Morgan Kaufmann Publishers Inc}},
 isbn = {1-55860-412-X}
}


@proceedings{.2002,
 year = {2002},
 title = {2002 IEEE International Conference on Robotics and Automation}
}


@proceedings{.2003,
 year = {2003},
 title = {IEEE International Conference on Robotics and Automation. IEEE ICRA 2003 Conference Proceedings}
}

@proceedings{.2005,
 year = {2005},
 title = {AIIDE}
}


@proceedings{.2005b,
 year = {2005},
 title = {2005 IEEE International Conference on Robotics and Automation}
}


@proceedings{.2006,
 year = {2006},
 title = {Proceedings of AAAI Workshop on Auction Mechanisms for Robot Coordination},
 publisher = {Citeseer}
}


@proceedings{.2006b,
 year = {2006},
 title = {AIIDE}
}


@proceedings{.2007,
 year = {2007},
 title = {2007 IEEE International Conference on Robotics and Automation}
}


@proceedings{.2008,
 year = {2008},
 title = {ICAPS}
}


@proceedings{.2008b,
 year = {2008},
 title = {2008 IEEE International Conference on Technologies for Practical Robot Applications (TePRA)}
}


@proceedings{.2008c,
 year = {2008},
 title = {3rd International Conference on Innovative Computing Information and Control}
}


@proceedings{.2010,
 year = {2010},
 title = {AAAI}
}


@proceedings{.2011,
 year = {2011},
 title = {2011 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS 2011)}
}


@proceedings{.2011b,
 year = {2011},
 title = {2011 IEEE International Conference on Automation Science and Engineering (CASE 2011)}
}


@proceedings{.2011c,
 year = {2011},
 title = {2011 5th International Conference on Automation, Robotics and Applications (ICARA 2011)}
}


@proceedings{.2012,
 year = {2012},
 title = {2012 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS 2012)}
}


@proceedings{.2012b,
 year = {2012},
 title = {2012 20th Mediterranean Conference on Control {\&} Automation (MED 2012)}
}


@proceedings{.2013,
 year = {2013},
 title = {Sixth Annual Symposium on Combinatorial Search}
}


@proceedings{.2013b,
 year = {2013},
 title = {2013 IEEE 18th Conference on Emerging Technologies {\&} Factory Automation (ETFA)}
}


@proceedings{.2014,
 year = {2014},
 title = {2014 IEEE Conference on Control Applications (CCA)}
}


@proceedings{.2014b,
 year = {2014},
 title = {Seventh Annual Symposium on Combinatorial Search}
}


@proceedings{.2014c,
 year = {2014},
 title = {Seventh Annual Symposium on Combinatorial Search}
}


@proceedings{.2015,
 year = {2015},
 title = {Proceedings of the Twenty-Ninth AAAI Workshops on Artificial Intelligence},
 isbn = {978-1-57735-712-4}
}


@proceedings{.2015b,
 year = {2015},
 title = {Eighth Annual Symposium on Combinatorial Search}
}


@proceedings{.2015c,
 year = {2015},
 title = {9th International Quality Conference}
}


@book{.2015d,
 year = {2015},
 title = {IROS 2015 Workshop on On-line decision-making in multi-robot coordination (DEMUR'15)}
}


@proceedings{.2016,
 year = {2016},
 title = {2016 IEEE International Conference on Automation Science and Engineering (CASE)},
 publisher = {IEEE},
 isbn = {978-1-5090-2409-4}
}


@proceedings{.2016b,
 year = {2016},
 title = {Proceedings of the 25th International Joint Conference on Artificial Intelligence (IJCAI) Workshop on Multi-Agent Path Finding}
}


@proceedings{.2016c,
 year = {2016},
 title = {2016 IEEE International Conference on Industrial Engineering and Engineering Management (IEEM)},
 publisher = {IEEE},
 isbn = {978-1-5090-3665-3}
}


@article{AbdAlgfoor.2015,
 author = {{Abd Algfoor}, Zeyad and Sunar, Mohd Shahrizal and Kolivand, Hoshang},
 year = {2015},
 title = {A Comprehensive Study on Pathfinding Techniques for Robotics and Video Games},
 pages = {1--11},
 volume = {2015},
 number = {2},
 issn = {1687-7047},
 journal = {International Journal of Computer Games Technology},
 doi = {10.1155/2015/736138}
}


@article{Amato.2005,
 author = {Amato, Francesco and Basile, Francesco and Carbone, Ciro and Chiacchio, Pasquale},
 year = {2005},
 title = {An approach to control automated warehouse systems},
 keywords = {Automated Storage and Retrieval Systems;Multi-Robot Task Allocation},
 pages = {1223--1241},
 volume = {13},
 number = {10},
 issn = {09670661},
 journal = {Control Engineering Practice},
 doi = {10.1016/j.conengprac.2004.10.017}
}


@article{Andriansyah.2011,
 author = {Andriansyah, R. and de Koning, W.W.H. and Jordan, R.M.E. and Etman, L.F.P. and Rooda, J. E.},
 year = {2011},
 title = {A process algebra based simulation model of a miniload-workstation order picking system},
 keywords = {Automated Storage and Retrieval Systems;Order Picking and Storage Assignment},
 pages = {292--300},
 volume = {62},
 number = {3},
 issn = {01663615},
 journal = {Computers in Industry},
 doi = {10.1016/j.compind.2010.09.005}
}


@article{Ang.2012,
 author = {Ang, Marcus and Lim, Yun Fong and Sim, Melvyn},
 year = {2012},
 title = {Robust Storage Assignment in Unit-Load Warehouses},
 pages = {2114--2130},
 volume = {58},
 number = {11},
 issn = {0025-1909},
 journal = {Management Science},
 doi = {10.1287/mnsc.1120.1543}
}

@article{archetti2003reoptimizing,
  title={Reoptimizing the traveling salesman problem},
  author={Archetti, Claudia and Bertazzi, Luca and Speranza, M Grazia},
  journal={Networks: An International Journal},
  volume={42},
  number={3},
  pages={154--159},
  year={2003},
  publisher={Wiley Online Library}
}

@misc{azadeh2017robotized,
	title={Robotized warehouse systems: Developments and research opportunities},
	author={Azadeh, Kaveh and de Koster, M and Roy, Debjit},
	note={Research paper (no. ERS-2017-009-LIS), ERIM Report Series Research in Management},
	year={2017}
}

@article{Azadnia.2013,
 author = {Azadnia, Amir Hossein and Taheri, Shahrooz and Ghadimi, Pezhman and {Mat Saman}, Muhamad Zameri and Wong, Kuan Yew},
 year = {2013},
 title = {Order batching in warehouses by minimizing total tardiness: a hybrid approach of weighted association rule mining and genetic algorithms},
 volume = {2013},
 journal = {The Scientific World Journal}
}


@article{Banker.1984,
 author = {Banker, R. D. and Charnes, A. and Cooper, W. W.},
 year = {1984},
 title = {Some Models for Estimating Technical and Scale Inefficiencies in Data Envelopment Analysis},
 pages = {1078--1092},
 volume = {30},
 number = {9},
 issn = {0025-1909},
 journal = {Management Science},
 doi = {10.1287/mnsc.30.9.1078}
}


@inproceedings{Barer.2014,
 author = {Barer, Max and Sharon, Guni and Stern, Roni and Felner, Ariel},
 title = {Suboptimal variants of the conflict-based search algorithm for the multi-agent pathfinding problem},
 booktitle = {Seventh Annual Symposium on Combinatorial Search},
 year = {2014}
}


@article{Bartholdi.2008,
 author = {Bartholdi, John J. and Hackman, Steven T.},
 year = {2008},
 title = {Allocating space in a forward pick area of a distribution center for small parts},
 pages = {1046--1053},
 volume = {40},
 number = {11},
 issn = {0740-817X},
 journal = {IIE Transactions},
 doi = {10.1080/07408170802167662}
}


@article{Bessenouci.2012,
 author = {Bessenouci, Hakim Nadir and Sari, Zaki and Ghomri, Lat{\'e}fa},
 year = {2012},
 title = {Metaheuristic based control of a flow rack automated storage retrieval system},
 pages = {1157--1166},
 volume = {23},
 number = {4},
 issn = {0956-5515},
 journal = {Journal of Intelligent Manufacturing},
 doi = {10.1007/s10845-010-0432-1}
}





@article{Bozer.2008,
 author = {Bozer, Y. A. and Kile, J. W.},
 year = {2008},
 title = {Order batching in walk-and-pick order picking systems},
 pages = {1887--1909},
 volume = {46},
 number = {7},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {10.1080/00207540600920850}
}


@article{Bukchin.2012,
 author = {Bukchin, Yossi and Khmelnitsky, Eugene and Yakuel, Pini},
 year = {2012},
 title = {Optimizing a dynamic order-picking process},
 keywords = {Order Picking and Storage Assignment},
 pages = {335--346},
 volume = {219},
 number = {2},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2011.12.041}
}


@article{Chan.2011,
 author = {Chan, Felix T.S. and Chan, H. K.},
 year = {2011},
 title = {Improving the productivity of order picking of a manual-pick and multi-level rack distribution warehouse through the implementation of class-based storage},
 pages = {2686--2700},
 volume = {38},
 number = {3},
 issn = {09574174},
 journal = {Expert Systems with Applications},
 doi = {10.1016/j.eswa.2010.08.058}
}


@article{Chen.2010,
 author = {Chen, Lu and Langevin, Andr{\'e} and Riopel, Diane},
 year = {2010},
 title = {The storage location assignment and interleaving problem in an automated storage/retrieval system with shared storage},
 pages = {991--1011},
 volume = {48},
 number = {4},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {10.1080/00207540802506218}
}


@article{Chen.2010b,
 author = {Chen, Chien-Ming and Gong, Yeming and de Koster, Ren{\'e} and {van Nunen}, Jo A.E.E.},
 year = {2010},
 title = {A Flexible Evaluative Framework for Order Picking Systems},
 pages = {70--82},
 volume = {19},
 number = {1},
 issn = {10591478},
 journal = {Production and Operations Management},
 doi = {10.1111/j.1937-5956.2009.01047.x}
}


@article{ChiaJane.2000,
 author = {{Chia Jane}, Chin},
 year = {2000},
 title = {Storage location assignment in a distribution center},
 pages = {55--71},
 volume = {30},
 number = {1},
 issn = {0960-0035},
 journal = {International Journal of Physical Distribution {\&} Logistics Management},
 doi = {10.1108/09600030010307984}
}


@inproceedings{Clark.2003,
 author = {Clark, C. M. and Rock, S. M. and Latombe, J.-C.},
 title = {Motion planning for multiple mobile robots using dynamic networks},
 pages = {4222--4227},
 booktitle = {IEEE International Conference on Robotics and Automation. IEEE ICRA 2003 Conference Proceedings},
 year = {2003},
 doi = {10.1109/ROBOT.2003.1242252}
}


@inproceedings{Cohen.2015,
 author = {Cohen, Liron and Uras, Tansel and Koenig, Sven},
 title = {Feasibility Study: Using Highways for Bounded-Suboptimal Multi-Agent Path Finding},
 booktitle = {Eighth Annual Symposium on Combinatorial Search},
 year = {2015}
}


@misc{Cohen.20170608,
 author = {Cohen, Liron and Wagner, Glenn and Kumar, T. K. Satish and Choset, Howie and Koenig, Sven},
 year = {2017},
 title = {Rapid Randomized Restarts for Multi-Agent Path Finding Solvers},
 url = {http://arxiv.org/pdf/1706.02794}
}


@article{Confessore.2013,
 author = {Confessore, Giuseppe and Fabiano, Marcello and Liotta, Giacomo},
 year = {2013},
 title = {A network flow based heuristic approach for optimising AGV movements},
 keywords = {AGV;Automated Material Handling System;Multi-Robot Path Planning (centralized);Multi-Robot Task Allocation},
 pages = {405--419},
 volume = {24},
 number = {2},
 issn = {0956-5515},
 journal = {Journal of Intelligent Manufacturing},
 doi = {10.1007/s10845-011-0612-7}
}


@book{Cooper.2007,
 author = {Cooper, William W. and Seiford, Lawrence M. and Tone, Kaoru},
 year = {2007},
 title = {Data Envelopment Analysis: A Comprehensive Text with Models, Applications, References and DEA-Solver Software},
 url = {http://dx.doi.org/10.1007/978-0-387-45283-8},
 keywords = {Datenanalyse;Online-Publikation},
 address = {Boston MA},
 edition = {Second Edition},
 publisher = {{Springer Science+Business Media LLC}},
 isbn = {9780387452838}
}


@article{Correa.2007,
 author = {Corr{\'e}a, Ayoub Insa and Langevin, Andr{\'e} and Rousseau, Louis-Martin},
 year = {2007},
 title = {Scheduling and routing of automated guided vehicles: A hybrid approach},
 pages = {1688--1707},
 volume = {34},
 number = {6},
 issn = {03050548},
 journal = {Computers {\&} Operations Research},
 doi = {10.1016/j.cor.2005.07.004}
}


@article{Dallari.2009,
 author = {Dallari, Fabrizio and Marchet, Gino and Melacini, Marco},
 year = {2009},
 title = {Design of order picking system},
 pages = {1--12},
 volume = {42},
 number = {1-2},
 issn = {0268-3768},
 journal = {The International Journal of Advanced Manufacturing Technology},
 doi = {10.1007/s00170-008-1571-9}
}


@inproceedings{DAndrea.2008,
 author = {D'Andrea, Raffaello and Wurman, Peter},
 title = {Future challenges of coordinating hundreds of autonomous vehicles in distribution facilities},
 pages = {80--83},
 booktitle = {2008 IEEE International Conference on Technologies for Practical Robot Applications (TePRA)},
 year = {2008},
 doi = {10.1109/TEPRA.2008.4686677}
}


@article{DAndrea.2012,
 author = {D'Andrea, Raffaello},
 year = {2012},
 title = {Guest Editorial: A Revolution in the Warehouse: A Retrospective on Kiva Systems and the Grand Challenges Ahead},
 pages = {638--639},
 volume = {9},
 number = {4},
 issn = {1545-5955},
 journal = {IEEE Transactions on Automation Science and Engineering},
 doi = {10.1109/TASE.2012.2214676}
}


@proceedings{Dunne.2014,
 year = {2014},
 title = {the 2014 ACM International Symposium},
 editor = {Dunne, Lucy and Martin, Tom and Beigl, Michael}
}


@article{Ene.2012,
 author = {Ene, Seval and {\"O}zt{\"u}rk, Nursel},
 year = {2012},
 title = {Storage location assignment and order picking optimization in the automotive industry},
 pages = {787--797},
 volume = {60},
 number = {5-8},
 issn = {0268-3768},
 journal = {The International Journal of Advanced Manufacturing Technology},
 doi = {10.1007/s00170-011-3593-y}
}


@inproceedings{Enright.2011,
 author = {Enright, John and Wurman, Peter R.},
 title = {Optimization and Coordinated Autonomy in Mobile Fulfillment Systems},
 keywords = {ApplicationDescription},
 editor = {{Sanem Sariel-Talay} and {Stephen F. Smith} and {Nilufer Onder}},
 booktitle = {Automated Action Planning for Autonomous Mobile Robots},
 year = {2011}
}


@article{Erol.2012,
 author = {Erol, Rizvan and Sahin, Cenk and Baykasoglu, Adil and Kaplanoglu, Vahit},
 year = {2012},
 title = {A multi-agent based approach to dynamic scheduling of machines and automated guided vehicles in manufacturing systems},
 pages = {1720--1732},
 volume = {12},
 number = {6},
 issn = {15684946},
 journal = {Applied Soft Computing},
 doi = {10.1016/j.asoc.2012.02.001}
}


@inproceedings{FangTang.2005,
 author = {{Fang Tang} and Parker, L. E.},
 title = {ASyMTRe: Automated Synthesis of Multi-Robot Task Solutions through Software Reconfiguration},
 pages = {1501--1508},
 booktitle = {2005 IEEE International Conference on Robotics and Automation},
 year = {2005},
 doi = {10.1109/ROBOT.2005.1570327}
}


@article{Fink.2014,
 author = {Fink, Andreas and Kliewer, Natalia and Mattfeld, Dirk and M{\"o}nch, Lars and Rothlauf, Franz and Schryen, Guido and Suhl, Leena and Vo{\ss}, Stefan},
 year = {2014},
 title = {Model-Based Decision Support in Manufacturing and Service Networks},
 pages = {17--24},
 volume = {6},
 number = {1},
 issn = {1867-0202},
 journal = {Business {\&} Information Systems Engineering},
 doi = {10.1007/s12599-013-0310-4}
}


@inproceedings{Fitzgerald.2014,
 author = {Fitzgerald, Tadhg and Malitsky, Yuri and O'Sullivan, Barry and Tierney, Kevin},
 title = {React: Real-time algorithm configuration through tournaments},
 booktitle = {Seventh Annual Symposium on Combinatorial Search},
 year = {2014}
}


@article{Fumi.2013,
 author = {Fumi, Andrea and Scarabotti, Laura and Schiraldi, Massimiliano M.},
 year = {2013},
 title = {The effect of slot-code optimization in warehouse order picking},
 url = {http://cdn.intechopen.com/pdfs/45486/InTech-The_effect_of_slot_code_optimization_in_warehouse_order_picking.pdf},
 keywords = {Order Picking and Storage Assignment},
 pages = {1--10},
 volume = {5},
 number = {20},
 journal = {International Journal of Engineering Business Management}
}


@article{Furmans.2009,
 author = {Furmans, Kai and Huber, Christian and Wisser, Jens},
 year = {2009},
 title = {Queueing Models for manual order picking systems with blocking},
 volume = {1},
 number = {01},
 journal = {Logistics Journal}
}


@article{Gagliardi.2012,
 author = {Gagliardi, Jean-Philippe and Renaud, Jacques and Ruiz, Angel},
 year = {2012},
 title = {On storage assignment policies for unit-load automated storage and retrieval systems},
 pages = {879--892},
 volume = {50},
 number = {3},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {10.1080/00207543.2010.543939}
}


@article{Gagliardi.2012b,
 author = {Gagliardi, Jean-Philippe and Renaud, Jacques and Ruiz, Angel},
 year = {2012},
 title = {Models for automated storage and retrieval systems: A literature review},
 pages = {7110--7125},
 volume = {50},
 number = {24},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {10.1080/00207543.2011.633234}
}


@inproceedings{Geramifard.2006,
 author = {Geramifard, Alborz and Chubak, Pirooz and Bulitko, Vadim},
 title = {Biased Cost Pathfinding},
 pages = {112--114},
 booktitle = {AIIDE},
 year = {2006}
}


@article{Gerkey.2004,
 author = {Gerkey, B. P.},
 year = {2004},
 title = {A Formal Analysis and Taxonomy of Task Allocation in Multi-Robot Systems},
 keywords = {Review Paper},
 pages = {939--954},
 volume = {23},
 number = {9},
 issn = {0278-3649},
 journal = {The International Journal of Robotics Research},
 doi = {10.1177/0278364904045564}
}


@article{Gu.2007,
 author = {Gu, Jinxiang and Goetschalckx, Marc and McGinnis, Leon F.},
 year = {2007},
 title = {Research on warehouse operation: A comprehensive review},
 pages = {1--21},
 volume = {177},
 number = {1},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2006.02.025}
}


@article{Gu.2010,
 author = {Gu, Jinxiang and Goetschalckx, Marc and McGinnis, Leon F.},
 year = {2010},
 title = {Research on warehouse design and performance evaluation: A comprehensive review},
 pages = {539--549},
 volume = {203},
 number = {3},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2009.07.031}
}


@inproceedings{Guo.2014,
 author = {Guo, Anhong and Starner, Thad and Raghu, Shashank and Xie, Xuwen and Ismail, Saad and Luo, Xiaohui and Simoneau, Joseph and Gilliland, Scott and Baumann, Hannes and Southern, Caleb},
 title = {A comparison of order picking assisted by head-up display (HUD), cart-mounted display (CMD), light, and paper pick list},
 pages = {71--78},
 editor = {Dunne, Lucy and Martin, Tom and Beigl, Michael},
 booktitle = {the 2014 ACM International Symposium},
 year = {2014},
 doi = {10.1145/2634317.2634321}
}


@article{Haneyah.2013,
 author = {Haneyah, S.W.A. and Schutten, J.M.J. and Schuur, P. C. and Zijm, W.H.M.},
 year = {2013},
 title = {Generic planning and control of automated material handling systems},
 keywords = {ApplicationDescription;Automated Storage and Retrieval Systems;Review Paper},
 pages = {177--190},
 volume = {64},
 number = {3},
 issn = {01663615},
 journal = {Computers in Industry},
 doi = {10.1016/j.compind.2012.11.003}
}


@book{Hannebauer.2001,
 year = {2001},
 title = {Balancing reactivity and social deliberation in multi-agent systems: From RoboCup to real-world applications},
 keywords = {Artificial intelligence;Fu{\ss}ball;Intelligence artificielle;Intelligent agents (Computer software);Konfrontation;Kooperation;Mehragentensystem;Probleml{\"o}sen;r{\'e}activit{\'e};Reaktives System;robotique;Selbst organisierendes System;sociologie communication;Soziales System;syst{\`e}me multi-agent;travail coop{\'e}ratif},
 address = {Berlin and New York},
 volume = {2103. Lecture notes in artificial intelligence},
 publisher = {Springer},
 isbn = {978-3-540-42327-0},
 series = {Lecture Notes in Computer Science},
 editor = {Hannebauer, Markus and Wendler, Jan and Pagello, Enrico},
 doi = {10.1007/3-540-44568-4}
}


@inproceedings{Hazard.2006,
 author = {Hazard, Christopher J. and Wurman, Peter R. and D'Andrea, Raffaello},
 title = {Alphabet Soup: A Testbed for Studying Resource Allocation in Multi-vehicle Systems},
 pages = {23--30},
 publisher = {Citeseer},
 booktitle = {Proceedings of AAAI Workshop on Auction Mechanisms for Robot Coordination},
 year = {2006}
}


@article{Henn.2012,
 author = {Henn, Sebastian},
 year = {2012},
 title = {Algorithms for on-line order batching in an order picking warehouse},
 keywords = {Order batching},
 pages = {2549--2563},
 volume = {39},
 number = {11},
 issn = {03050548},
 journal = {Computers {\&} Operations Research},
 doi = {10.1016/j.cor.2011.12.019}
}


@article{Henn.2012b,
 author = {Henn, Sebastian and W{\"a}scher, Gerhard},
 year = {2012},
 title = {Tabu search heuristics for the order batching problem in manual order picking systems},
 keywords = {Order batching;Order Picking and Storage Assignment},
 pages = {484--494},
 volume = {222},
 number = {3},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2012.05.049}
}


@article{HernandezMartinez.2014,
 author = {Hernandez-Martinez, Eduardo G. and Foyo-Valdes, Sergio A. and Puga-Velazquez, Erika S. and Meda-Campa{\~n}a, Jes{\'u}s A.},
 year = {2014},
 title = {Hybrid Architecture for Coordination of AGVs in FMS},
 keywords = {AGV;Multi-Robot Path Planning (centralized);Multi-Robot Task Allocation},
 pages = {41},
 volume = {11},
 issn = {1729-8806},
 journal = {International Journal of Advanced Robotic Systems}
}


@article{Herold.2005,
 author = {Herold, Martin and Couclelis, Helen and Clarke, Keith C.},
 year = {2005},
 title = {The role of spatial metrics in the analysis and modeling of urban land use change},
 pages = {369--399},
 volume = {29},
 number = {4},
 issn = {01989715},
 journal = {Computers, Environment and Urban Systems},
 doi = {10.1016/j.compenvurbsys.2003.12.001}
}


@article{HerreroPerez.2010,
 author = {Herrero-Perez, D. and Martinez-Barbera, H.},
 year = {2010},
 title = {Modeling Distributed Transportation Systems Composed of Flexible Automated Guided Vehicles in Flexible Manufacturing Systems},
 keywords = {AGV;Automated Material Handling System;Multi-Robot Path Planning (decentralized);Multi-Robot Task Allocation},
 pages = {166--180},
 volume = {6},
 number = {2},
 issn = {1551-3203},
 journal = {IEEE Transactions on Industrial Informatics},
 doi = {10.1109/TII.2009.2038691}
}


@misc{Hoffman.2013,
 author = {Hoffman, A. E. and Mountz, M. C. and Barbehenn, M. T. and Allard, J. R. and Kimmel, M. E. and Santini, F. and Decker, M. H. and D'Andrea, R. and Wurman, P. R.},
 year = {2013},
 title = {System and method for inventory management using mobile drive units},
 url = {https://www.google.com/patents/US20130103552}
}


@book{Hompel.2010,
 author = {Hompel, Michael and Schmidt, Thorsten},
 year = {2010},
 title = {Warehouse Management: Organisation und Steuerung von Lager- und Kommissioniersystemen},
 address = {Berlin, Heidelberg},
 publisher = {{Springer -Verlag Berlin Heidelberg}},
 isbn = {3642031846},
 series = {VDI-Buch}
}


@article{Hsieh.2001,
 author = {Hsieh, S. and Tsai, K.-C.},
 year = {2001},
 title = {A BOM Oriented Class-Based Storage Assignment in an Automated Storage/Retrieval System},
 pages = {683--691},
 volume = {17},
 number = {9},
 issn = {0268-3768},
 journal = {The International Journal of Advanced Manufacturing Technology},
 doi = {10.1007/s001700170134}
}


@article{Hsieh.2011,
 author = {Hsieh, Ling-Feng and Huang, Yi-Chen},
 year = {2011},
 title = {New batch construction heuristics to optimise the performance of order picking systems},
 pages = {618--630},
 volume = {131},
 number = {2},
 issn = {09255273},
 journal = {International Journal of Production Economics},
 doi = {10.1016/j.ijpe.2011.02.006}
}


@article{Hsu.2005,
 author = {Hsu, Chih-Ming and Chen, Kai-Ying and Chen, Mu-Chen},
 year = {2005},
 title = {Batching orders in warehouses by minimizing travel distance with genetic algorithms},
 pages = {169--178},
 volume = {56},
 number = {2},
 issn = {01663615},
 journal = {Computers in Industry},
 doi = {10.1016/j.compind.2004.06.001}
}


@article{Huang.2015,
 author = {Huang, George Q. and Chen, Michael Z. Q. and Pan, Jia},
 year = {2015},
 title = {Robotics in ecommerce logistics},
 pages = {1--10},
 issn = {1023-697X},
 journal = {HKIE Transactions},
 doi = {10.1080/1023697X.2015.1043960}
}


@article{II.2000,
 author = {II, CHARLES G. PETERSEN},
 year = {2000},
 title = {AN EVALUATION OF ORDER PICKING POLICIES FOR MAIL ORDER COMPANIES},
 pages = {319--335},
 volume = {9},
 number = {4},
 issn = {10591478},
 journal = {Production and Operations Management},
 doi = {10.1111/j.1937-5956.2000.tb00461.x}
}


@incollection{Iocchi.2001,
 author = {Iocchi, Luca and Nardi, Daniele and Salerno, Massimiliano},
 title = {Reactivity and Deliberation: A Survey on Multi-Robot Systems},
 pages = {9--32},
 volume = {2103},
 publisher = {Springer},
 isbn = {978-3-540-42327-0},
 series = {Lecture Notes in Computer Science},
 editor = {Hannebauer, Markus and Wendler, Jan and Pagello, Enrico},
 booktitle = {Balancing reactivity and social deliberation in multi-agent systems},
 year = {2001},
 address = {Berlin and New York},
 doi = {10.1007/3-540-44568-4{\textunderscore }2}
}


@article{Jones.2011,
 author = {Jones, E. Gil and Dias, M. Bernardine and Stentz, Anthony},
 year = {2011},
 title = {Time-extended multi-robot coordination for domains with intra-path constraints},
 pages = {41--56},
 volume = {30},
 number = {1},
 issn = {0929-5593},
 journal = {Autonomous Robots},
 doi = {10.1007/s10514-010-9202-3}
}


@book{Junemann.1989,
 author = {J{\"u}nemann, R. and Pfohl, H.-C. and J{\"u}nemann, Reinhardt},
 year = {1989},
 title = {Materialflu{\ss} und Logistik},
 address = {Berlin, Heidelberg},
 publisher = {{Springer Berlin Heidelberg}},
 isbn = {978-3-540-51225-7},
 doi = {10.1007/978-3-662-08532-5}
}


@inproceedings{Kalinovcic.2011,
 author = {Kalinovcic, Luka and Petrovic, Tamara and Bogdan, Stjepan and Bobanac, Vedran},
 title = {Modified Banker's algorithm for scheduling in multi-AGV systems},
 keywords = {AGV;Multi-Robot Path Planning (centralized)},
 pages = {351--356},
 booktitle = {2011 IEEE International Conference on Automation Science and Engineering (CASE 2011)},
 year = {2011},
 doi = {10.1109/CASE.2011.6042433}
}


@inproceedings{Kamagaew.2011,
 author = {Kamagaew, Andreas and Stenzel, Jonas and Nettstrater, Andreas and ten Hompel, Michael},
 title = {Concept of Cellular Transport Systems in facility logistics},
 pages = {40--45},
 booktitle = {2011 5th International Conference on Automation, Robotics and Applications (ICARA 2011)},
 year = {2011},
 doi = {10.1109/ICARA.2011.6144853}
}


@article{Kim.2003,
 author = {Kim, Byung-In and Heragu, S. S. and Graves, R. J. and {St. Onge}, A.},
 year = {2003},
 title = {A hybrid scheduling and control system architecture for warehouse management},
 keywords = {Automated Storage and Retrieval Systems;Multi-Robot Task Allocation;Order batching},
 pages = {991--1001},
 volume = {19},
 number = {6},
 issn = {1042-296X},
 journal = {IEEE Transactions on Robotics and Automation},
 doi = {10.1109/TRA.2003.819735}
}


@article{Kirks.2012,
 author = {Kirks, Thomas and Stenzel, Jonas and Kamagaew, Andreas and ten Hompel, Michael},
 year = {2012},
 title = {Zellulare Transportfahrzeuge f{\"u}r flexible und wandelbare Intralogistiksysteme},
 pages = {1},
 volume = {2192},
 number = {9084},
 journal = {Logistics Journal}
}


@inproceedings{Kolhe.2012,
 author = {Kolhe, Pushkar and Christensen, Henrik I.},
 title = {Finding graph topologies for feasible multirobot motion planning},
 pages = {3754--3759},
 booktitle = {2012 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS 2012)},
 year = {2012},
 doi = {10.1109/IROS.2012.6386147}
}


@article{Korsah.2013,
 author = {Korsah, G. A. and Stentz, A. and Dias, M. B.},
 year = {2013},
 title = {A comprehensive taxonomy for multi-robot task allocation},
 keywords = {Review Paper;Taxonomy},
 pages = {1495--1512},
 volume = {32},
 number = {12},
 issn = {0278-3649},
 journal = {The International Journal of Robotics Research},
 doi = {10.1177/0278364913496484}
}

@incollection{Kovacevic.2015,
 author = {Kova{\v{c}}evi{\'c}, Nikola and Eri{\'c}, Milan and Aleksi{\'c}, Nata{\v{s}}a},
 title = {The use of automatic guided vehicles in order to increase the quality of the process of storage of goods},
 booktitle = {9th International Quality Conference 2015}
}


@article{Kovacs.2011,
 author = {Kov{\'a}cs, Andr{\'a}s},
 year = {2011},
 title = {Optimizing the storage assignment in a warehouse served by milkrun logistics},
 pages = {312--318},
 volume = {133},
 number = {1},
 issn = {09255273},
 journal = {International Journal of Production Economics},
 doi = {10.1016/j.ijpe.2009.10.028}
}


@inproceedings{Krontiris.2013,
 author = {Krontiris, Athanasios and Luna, Ryan and Bekris, Kostas E.},
 title = {From feasibility tests to path planners for multi-agent pathfinding},
 booktitle = {Sixth Annual Symposium on Combinatorial Search},
 year = {2013}
}


@article{Lamballais.2016,
 author = {Lamballais, T. and Roy, D. and de Koster, M.B.M.},
 year = {2016},
 title = {Estimating performance in a Robotic Mobile Fulfillment System},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2016.06.063}
}


@article{LauH.Y.K..2008,
 author = {{Lau, H. Y. K.} and Woo, S. O.},
 year = {2008},
 title = {An agent-based dynamic routing strategy for automated material handling systems},
 keywords = {Automated Material Handling System},
 pages = {269--288},
 volume = {21},
 number = {3},
 issn = {0951-192X},
 journal = {International Journal of Computer Integrated Manufacturing},
 doi = {10.1080/09511920701241624}
}


@article{LeAnh.2006,
 author = {Le-Anh, Tuan and de Koster, Ren{\'e}},
 year = {2006},
 title = {A review of design and control of automated guided vehicle systems},
 keywords = {AGV;Review Paper},
 pages = {1--23},
 volume = {171},
 number = {1},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2005.01.036}
}


@inproceedings{Li.2008,
 author = {Li, Meijuan and Chen, Xuebo and Liu, Chenqi},
 title = {Pareto and Niche Genetic Algorithm for Storage Location Assignment Optimization Problem},
 pages = {465},
 booktitle = {3rd International Conference on Innovative Computing Information and Control},
 year = {2008},
 doi = {10.1109/ICICIC.2008.655}
}


@article{Li.2013,
 author = {Li, Hanqing and Ru, Yihong and Han, Jihua and Xu, Weiyang},
 year = {2013},
 title = {What Makes a Difference? An Evaluation and Identification Approach to Distribution Center Productivity Using DEA},
 pages = {8308--8312},
 volume = {12},
 number = {24},
 issn = {18125638},
 journal = {Information Technology Journal},
 doi = {10.3923/itj.2013.8308.8312}
}


@article{Li.2017,
 author = {Li, Z. P. and Zhang, J. L. and Zhang, H. J. and Hua, G. W.},
 year = {2017},
 title = {Optimal selection of movable shelves under cargo-to-person picking mode},
 pages = {145--156},
 number = {Vol. 16 Issue 1},
 journal = {International Journal of Simulation Modelling (IJSIMM)}
}


@inproceedings{Luna.2011,
 author = {Luna, Ryan and Bekris, Kostas E.},
 title = {Efficient and complete centralized multi-robot path planning},
 keywords = {Multi-Robot Path Planning (centralized)},
 pages = {3268--3275},
 booktitle = {2011 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS 2011)},
 year = {2011},
 doi = {10.1109/IROS.2011.6095085}
}


@inproceedings{Ma.2016,
 author = {Ma, Hang and Koenig, Sven and Ayanian, Nora and Cohen, Liron and Hoenig, Wolfgang and Kumar, T. SatishK. and Uras, Tansel and Xu, Hong and Tovey, Craig and Sharon, Guni},
 title = {Overview: Generalizations of Multi-Agent Path Finding to Real-World Scenarios},
 booktitle = {Proceedings of the 25th International Joint Conference on Artificial Intelligence (IJCAI) Workshop on Multi-Agent Path Finding},
 year = {2016}
}


@incollection{Ma.2016b,
 author = {Ma, Hang and Koenig, Sven},
 title = {Optimal Target Assignment and Path Finding for Teams of Agents},
 url = {http://dl.acm.org/ft_gateway.cfm?id=2937092&type=pdf},
 keywords = {heuristic search;kiva (amazon robotics) systems;multi-agent path finding;multi-robot path finding;network flow;path planning;robotics;target assignment;team work;warehouse automation},
 editor = {Thangarajah, J. and Tuyls, K. and Jonker, C. and Marsella, S.},
 booktitle = {Proceedings of the 15th International Conference on Autonomous Agents and Multiagent Systems (AAMAS 2016)},
 year = {2016}
}


@article{Manor.2016,
 author = {Manor, Gil and Rimon, Elon},
 year = {2016},
 title = {The speed graph method: Pseudo time optimal navigation among obstacles subject to uniform braking safety constraints},
 issn = {0929-5593},
 journal = {Autonomous Robots},
 doi = {10.1007/s10514-015-9538-9}
}


@article{Manzini.2006,
 author = {Manzini, Riccardo and Gamberi, Mauro and Regattieri, Alberto},
 year = {2006},
 title = {Design and control of an AS/RS},
 pages = {766--774},
 volume = {28},
 number = {7-8},
 issn = {0268-3768},
 journal = {The International Journal of Advanced Manufacturing Technology},
 doi = {10.1007/s00170-004-2427-6}
}


@book{Manzini.2012,
 year = {2012},
 title = {Warehousing in the Global Supply Chain},
 address = {London},
 publisher = {{Springer London}},
 isbn = {978-1-4471-2273-9},
 editor = {Manzini, Riccardo},
 doi = {10.1007/978-1-4471-2274-6}
}


@article{MartinezBarbera.2010,
 abstract = {The research presented in this paper approaches the issue of navigation using an automated guided vehicle (AGV) in industrial environments. The work describes the navigation system of a flexible AGV intended for operation in partially structured warehouses and with frequent changes in the floor plant layout. This is achieved by incorporating a high degree of on-board autonomy and by decreasing the amount of manual work required by the operator when establishing the a priori knowledge of the environment. The AGV's autonomy consists of the set of automatic tasks, such as planner, perception, path planning and path tracking, that the industrial vehicle must perform to accomplish the task required by the operator. The integration of these techniques has been tested in a real AGV working on an industrial warehouse environment.},
 author = {Mart{\'i}nez-Barber{\'a}, H. and Herrero-P{\'e}rez, D.},
 year = {2010},
 title = {Autonomous navigation of an automated guided vehicle in industrial environments},
 url = {http://www.sciencedirect.com/science/article/pii/S0736584509000994},
 keywords = {Multi-Robot Path Planning (decentralized)},
 pages = {296--311},
 volume = {26},
 number = {4},
 issn = {0736-5845},
 journal = {Robotics and Computer-Integrated Manufacturing},
 doi = {10.1016/j.rcim.2009.10.003}
}


@article{Matusiak.2014,
 author = {Matusiak, Marek and de Koster, Ren{\'e} and Kroon, Leo and Saarinen, Jari},
 year = {2014},
 title = {A fast simulated annealing method for batching precedence-constrained customer orders in a warehouse},
 pages = {968--977},
 volume = {236},
 number = {3},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2013.06.001}
}


@incollection{MendesFilho.2015,
 author = {{Mendes Filho}, Jos{\'e} M. and Lucet, Eric},
 title = {Multi-robot motion planning:~A~modified receding horizon approach for reaching goal states},
 booktitle = {IROS 2015 Workshop on On-line decision-making in multi-robot coordination (DEMUR'15)},
 year = {2015}
}


@article{Meneghetti.2013,
 author = {Meneghetti, Antonella and Monti, Luca},
 year = {2013},
 title = {Sustainable storage assignment and dwell-point policies for automated storage and retrieval systems},
 pages = {511--520},
 volume = {24},
 number = {6},
 issn = {0953-7287},
 journal = {Production Planning {\&} Control},
 doi = {10.1080/09537287.2011.637525}
}


@inproceedings{Merschformann.2015,
 author = {Merschformann, Marius},
 title = {Algorithm Configuration Applied to Heuristics for Three-Dimensional Knapsack Problems in Air Cargo},
 isbn = {978-1-57735-712-4},
 booktitle = {Proceedings of the Twenty-Ninth AAAI Workshops on Artificial Intelligence},
 year = {2015}
}


@ARTICLE{Merschformann.2017,
   author = {{Merschformann}, M. and {Xie}, L. and {Erdmann}, D.},
    title = "{Multi-Agent Path Finding with Kinematic Constraints for Robotic Mobile Fulfillment Systems}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {http://arxiv.org/abs/1706.09347},
 primaryClass = "cs.AI",
 keywords = {Computer Science - Artificial Intelligence, Computer Science - Robotics},
     year = 2017,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170609347M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Moon.2001,
 author = {Moon, G. and Kim, G.-P.},
 year = {2001},
 title = {Effects of relocation to AS/RS storage location policy with production quantity variation},
 pages = {1--13},
 volume = {40},
 number = {1-2},
 issn = {03608352},
 journal = {Computers {\&} Industrial Engineering},
 doi = {10.1016/S0360-8352(00)00005-X}
}


@article{Muppani.2008,
 author = {Muppani, Venkata Reddy and Adil, Gajendra Kumar},
 year = {2008},
 title = {A branch and bound algorithm for class based storage location assignment},
 pages = {492--507},
 volume = {189},
 number = {2},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2007.05.050}
}


@article{Nam.2015,
 author = {Nam, Changjoo and Shell, Dylan A.},
 year = {2015},
 title = {Assignment Algorithms for Modeling Resource Contention in Multirobot Task Allocation},
 pages = {1--12},
 issn = {1545-5955},
 journal = {IEEE Transactions on Automation Science and Engineering},
 doi = {10.1109/TASE.2015.2415514}
}


@article{P.Raja.2012,
 author = {Raja, P. and Pugazhenthi, S.},
 year = {2012},
 title = {Optimal path planning of mobile robots: A review},
 volume = {7},
 number = {9},
 issn = {19921950},
 journal = {International Journal of the Physical Sciences},
 doi = {10.5897/IJPS11.1745}
}


@book{Paias.2016,
 year = {2016},
 title = {Computational Logistics: 7th International Conference, Iccl 2016, Lisbon, Portugal, September 7-9, 2016, Proceedings},
 address = {Cham},
 publisher = {{Springer-Verlag New York Inc}},
 isbn = {978-3-319-44895-4},
 series = {Lecture Notes in Computer Science},
 editor = {Paias, Ana and Ruthmair, Mario and Vo{\ss}, Stefan},
 doi = {10.1007/978-3-319-44896-1}
}


@article{Pan.1995,
 author = {Pan, C. and {Liu S.}},
 year = {1995},
 title = {A comparative study of order batching algorithms},
 pages = {691--700},
 volume = {23},
 number = {6},
 issn = {03050483},
 journal = {Omega},
 doi = {10.1016/0305-0483(95)00038-0}
}


@article{Pan.2008,
 author = {Pan, Jason Chao-Hsien and Shih, Po-Hsun},
 year = {2008},
 title = {Evaluation of the throughput of a multiple-picker order picking system with congestion consideration},
 pages = {379--389},
 volume = {55},
 number = {2},
 issn = {03608352},
 journal = {Computers {\&} Industrial Engineering},
 doi = {10.1016/j.cie.2008.01.002}
}


@article{Pan.2009,
 author = {Pan, Jason Chao-Hsien and Wu, Ming-Hung},
 year = {2009},
 title = {A study of storage assignment problem for an order picking line in a pick-and-pass warehousing system},
 pages = {261--268},
 volume = {57},
 number = {1},
 issn = {03608352},
 journal = {Computers {\&} Industrial Engineering},
 doi = {10.1016/j.cie.2008.11.026}
}


@article{Park.2006,
 author = {Park, Byung Chun and Foley, Robert D. and Frazelle, Edward H.},
 year = {2006},
 title = {Performance of miniload systems with two-class storage},
 pages = {144--155},
 volume = {170},
 number = {1},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2004.07.057}
}


@article{Petersen.2004,
 author = {Petersen, Charles G. and Aase, Gerald},
 year = {2004},
 title = {A comparison of picking, storage, and routing policies in manual order picking},
 pages = {11--19},
 volume = {92},
 number = {1},
 issn = {09255273},
 journal = {International Journal of Production Economics},
 doi = {10.1016/j.ijpe.2003.09.006}
}


@article{Petersen.2004b,
 author = {Petersen, Charles G. and Aase, Gerald R. and Heiser, Daniel R.},
 year = {2004},
 title = {Improving order-picking performance through the implementation of class-based storage},
 pages = {534--544},
 volume = {34},
 number = {7},
 journal = {International Journal of Physical Distribution {\&} Logistics Management}
}


@inproceedings{Petrovic.2014,
 author = {Petrovic, Tamara},
 title = {Path assignment and resource allocation control in reconfigurable multi-vehicle system},
 pages = {1789--1794},
 booktitle = {2014 IEEE Conference on Control Applications (CCA)},
 year = {2014},
 doi = {10.1109/CCA.2014.6981572}
}


@article{Pillac.2013,
 author = {Pillac, Victor and Gendreau, Michel and Gu{\'e}ret, Christelle and Medaglia, Andr{\'e}s L.},
 year = {2013},
 title = {A review of dynamic vehicle routing problems},
 keywords = {Review Paper},
 pages = {1--11},
 volume = {225},
 number = {1},
 journal = {European journal of operational research : EJOR}
}


@article{Reaidy.2015,
 author = {Reaidy, Paul J. and Gunasekaran, Angappa and Spalanzani, Alain},
 year = {2015},
 title = {Bottom-up approach based on Internet of Things for order fulfillment in a collaborative warehousing environment},
 pages = {29--40},
 volume = {159},
 issn = {09255273},
 journal = {International Journal of Production Economics},
 doi = {10.1016/j.ijpe.2014.02.017}
}


@inproceedings{RibasXirgo.2013,
 author = {Ribas-Xirgo, Lluis and Chaile, Ismael F.},
 title = {Multi-agent-based controller architecture for AGV systems},
 keywords = {AGV;Architecture Description},
 pages = {1--4},
 booktitle = {2013 IEEE 18th Conference on Emerging Technologies {\&} Factory Automation (ETFA)},
 year = {2013},
 doi = {10.1109/ETFA.2013.6648084}
}


@book{Richard.2008,
 author = {Richard, Hans Albert and Sander, Manuela},
 year = {2008},
 title = {Technische Mechanik - Dynamik: Grundlagen - effektiv und anwendungsnah},
 keywords = {Dynamik},
 address = {Wiesbaden},
 edition = {1. Aufl.},
 publisher = {Vieweg},
 isbn = {9783528039950},
 series = {Viewegs Fachb{\"u}cher der Technik}
}


@article{Roodbergen.2009,
 author = {Roodbergen, Kees Jan and Vis, Iris F.A.},
 year = {2009},
 title = {A survey of literature on automated storage and retrieval systems},
 keywords = {Automated Storage and Retrieval Systems;Multi-Robot Task Allocation;Review Paper},
 pages = {343--362},
 volume = {194},
 number = {2},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2008.01.038}
}


@article{Roodbergen.2014,
 author = {Roodbergen, Kees Jan and Vis, Iris F.A. and Taylor, G. Don},
 year = {2014},
 title = {Simultaneous determination of warehouse layout and control policies},
 pages = {3306--3326},
 volume = {53},
 number = {11},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {10.1080/00207543.2014.978029}
}


@article{Ruben.1999,
 author = {Ruben, Robert A. and Jacobs, F. Robert},
 year = {1999},
 title = {Batch Construction Heuristics and Storage Assignment Strategies for Walk/Ride and Pick Systems},
 pages = {575--596},
 volume = {45},
 number = {4},
 issn = {0025-1909},
 journal = {Management Science},
 doi = {10.1287/mnsc.45.4.575}
}


@proceedings{SanemSarielTalay.2011,
 year = {2011},
 title = {Automated Action Planning for Autonomous Mobile Robots},
 editor = {{Sanem Sariel-Talay} and {Stephen F. Smith} and {Nilufer Onder}}
}


@inproceedings{Schieweck.2016,
 author = {Schieweck, S. and Kern-Isberner, G. and ten Hompel, M.},
 title = {Using answer set programming in an order-picking system with cellular transport vehicles},
 pages = {1600--1604},
 publisher = {IEEE},
 isbn = {978-1-5090-3665-3},
 booktitle = {2016 IEEE International Conference on Industrial Engineering and Engineering Management (IEEM)},
 year = {2016},
 doi = {10.1109/IEEM.2016.7798147}
}


@article{Sharon.2015,
 author = {Sharon, Guni and Stern, Roni and Felner, Ariel and Sturtevant, Nathan R.},
 year = {2015},
 title = {Conflict-based search for optimal multi-agent pathfinding},
 pages = {40--66},
 volume = {219},
 issn = {00043702},
 journal = {Artificial Intelligence},
 doi = {10.1016/j.artint.2014.11.006}
}


@book{Sherman.2006,
 author = {Sherman, H. David and Joe, Zhu},
 year = {2006},
 title = {Service Productivity Management},
 publisher = {{Springer US}},
 isbn = {978-0-387-33211-6},
 doi = {10.1007/0-387-33231-6}
}


@article{Silver.2005,
 author = {Silver, David},
 title = {Cooperative Pathfinding},
 journal = {Proceedings of the First Artificial Intelligence and Interactive Digital
               Entertainment Conference (2005)},
url = {http://www.aaai.org/Papers/AIIDE/2005/AIIDE05-020.pdf},
}


@article{SmolicRocak.2010,
 author = {Smolic-Rocak, N. and Bogdan, S. and Kovacic, Z. and Petrovic, T.},
 year = {2010},
 title = {Time Windows Based Dynamic Routing in Multi-AGV Systems},
 keywords = {AGV;Multi-Robot Path Planning (centralized)},
 pages = {151--155},
 volume = {7},
 number = {1},
 issn = {1545-5955},
 journal = {IEEE Transactions on Automation Science and Engineering},
 doi = {10.1109/TASE.2009.2016350}
}


@article{Sprunk.2016,
 author = {Sprunk, Christoph and Lau, Boris and Pfaff, Patrick and Burgard, Wolfram},
 year = {2016},
 title = {An accurate and efficient navigation system for omnidirectional robots in industrial environments},
 issn = {0929-5593},
 journal = {Autonomous Robots},
 doi = {10.1007/s10514-016-9557-1}
}


@inproceedings{Standley.2010,
 author = {Standley, Trevor Scott},
 title = {Finding Optimal Solutions to Cooperative Pathfinding Problems},
 pages = {28--29},
 volume = {1},
 booktitle = {AAAI},
 year = {2010}
}


@inproceedings{Stavrou.2012,
 author = {Stavrou, Demetris and Panayiotou, Christos},
 title = {Task assignment and agent coordination in a warehouse environment},
 pages = {1341--1346},
 booktitle = {2012 20th Mediterranean Conference on Control {\&} Automation (MED 2012)},
 year = {2012},
 doi = {10.1109/MED.2012.6265825}
}


@inproceedings{Stenzel.2016,
 author = {Stenzel, Jonas and Luensch, Dennis},
 title = {Concept of decentralized cooperative path conflict resolution for heterogeneous mobile robots},
 pages = {715--720},
 publisher = {IEEE},
 isbn = {978-1-5090-2409-4},
 booktitle = {2016 IEEE International Conference on Automation Science and Engineering (CASE)},
 year = {2016},
 doi = {10.1109/COASE.2016.7743472}
}


@phdthesis{Stowe.2016,
 abstract = {In 2003 Kiva Systems (now Amazon Robotics) introduced a new type material handling automation to the world. The system is based on the principle that the physical infrastructure that contains inventory should be mobile. Kiva achieved this remarkable advancement by employing a fleet of robots to move shelving to human operators. Broadly, these types of systems are defined in the literature as multi-agent robotic systems. Amazon acquired Kiva Systems in 2012 to incorporate the technology into their operations. The goal of this thesis is to optimize the throughput of warehouses employing multi-agent robotic automation. It is assumed that extracting inventory from the automated system is the limiting factor in maximizing throughput (i.e. downstream process are unconstrained). Two strategies are advocated: 1) performing velocity segregation of inventory within the automation via a bifurcation between fast selling and slow selling inventory, 2) maximizing pick rates through policies that increase worker retention. It will be shown that velocity segregation increases machine efficiency by increasing the efficiency of delivering inventory to human operators. This assertion will be investigated by developing a theoretical understanding of how inventory velocity impacts machine efficiency and simulating different types of stow strategies impact on system efficiency. It is estimated that some stow strategies can increase machine efficiency by as much as 30{\%}. It will also be shown that the number of man-hours worked by inexperienced pickers explains practically all of the variability of aggregate pick cycle times and hence pick rates, which motivates the argument for worker retention. Together, these two modifications are estimated to increase throughput by 10{\%} over current baseline.},
 author = {Stowe, James DeWitt},
 year = {2016},
 title = {Throughput optimization of multi-agent robotic automated warehouses},
 url = {http://dspace.mit.edu/bitstream/1721.1/104388/1/958267045-MIT.pdf},
 keywords = {and Society;and Society.;Engineering Systems Division;Engineering Systems Division.;Institute for Data;Leaders for Global Operations Program;Leaders for Global Operations Program.;Sloan School of Management;Sloan School of Management.;Systems;Thesis},
 school = {{Massachusetts Institute of Technology}},
 type = {Master Thesis}
}


@misc{Surynek.2016,
 author = {Surynek, Pavel},
 year = {2016},
 title = {Makespan Optimal Solving of Cooperative Path-Finding via Reductions to Propositional Satisfiability},
 url = {http://arxiv.org/pdf/1610.05452}
}


@inproceedings{Tang.2007,
 author = {Tang, Fang and Parker, Lynne E.},
 title = {A Complete Methodology for Generating Multi-Robot Task Solutions using ASyMTRe-D and Market-Based Task Allocation},
 pages = {3351--3358},
 booktitle = {2007 IEEE International Conference on Robotics and Automation},
 year = {2007},
 doi = {10.1109/ROBOT.2007.363990}
}


@article{Tappia.2017,
 author = {Tappia, Elena and Roy, Debjit and de Koster, Ren{\'e} and Melacini, Marco},
 year = {2017},
 title = {Modeling, Analysis, and Design Insights for Shuttle-Based Compact Storage Systems},
 pages = {269--295},
 volume = {51},
 number = {1},
 issn = {0041-1655},
 journal = {Transportation Science},
 doi = {\url{10.1287/trsc.2016.0699}}
}


@book{Thangarajah.2016,
 year = {2016},
 title = {Proceedings of the 15th International Conference on Autonomous Agents and Multiagent Systems (AAMAS 2016)},
 editor = {Thangarajah, J. and Tuyls, K. and Jonker, C. and Marsella, S.}
}


@article{Turpin.2014,
 author = {Turpin, M. and Michael, N. and Kumar, V.},
 year = {2014},
 title = {CAPT: Concurrent assignment and planning of trajectories for multiple robots},
 keywords = {Multi-Robot Path Planning (centralized);Multi-Robot Path Planning (decentralized);Multi-Robot Task Allocation},
 pages = {98--112},
 volume = {33},
 number = {1},
 issn = {0278-3649},
 journal = {The International Journal of Robotics Research},
 doi = {10.1177/0278364913515307}
}


@article{Turpin.2014b,
 author = {Turpin, Matthew and Mohta, Kartik and Michael, Nathan and Kumar, Vijay},
 year = {2014},
 title = {Goal assignment and trajectory planning for large teams of interchangeable robots},
 pages = {401--415},
 volume = {37},
 number = {4},
 issn = {0929-5593},
 journal = {Autonomous Robots},
 doi = {10.1007/s10514-014-9412-1}
}


@article{vandenBergJeroenP..2000,
 author = {{van den Berg, Jeroen P.} and Gademann, A.J.R.M.},
 year = {2000},
 title = {Simulation study of an automated storage/retrieval system},
 pages = {1339--1356},
 volume = {38},
 number = {6},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {10.1080/002075400188889}
}


@incollection{vanGils.2016,
 author = {{van Gils}, Teun and Braekers, Kris and Ramaekers, Katrien and Depaire, Beno{\^i}t and Caris, An},
 title = {Improving Order Picking Efficiency by Analyzing Combinations of Storage, Batching, Zoning, and Routing Policies},
 pages = {427--442},
 volume = {9855},
 publisher = {{Springer-Verlag New York Inc}},
 isbn = {978-3-319-44895-4},
 series = {Lecture Notes in Computer Science},
 editor = {Paias, Ana and Ruthmair, Mario and Vo{\ss}, Stefan},
 booktitle = {Computational Logistics},
 year = {2016},
 address = {Cham},
 doi = {10.1007/978-3-319-44896-1{\textunderscore }28}
}


@incollection{Vasili.2012,
 author = {Vasili, M. R. and Tang, Sai Hong and Vasili, Mehdi},
 title = {Automated Storage and Retrieval Systems: A Review on Travel Time Models and Control Policies},
 pages = {159--209},
 publisher = {{Springer London}},
 isbn = {978-1-4471-2273-9},
 editor = {Manzini, Riccardo},
 booktitle = {Warehousing in the Global Supply Chain},
 year = {2012},
 address = {London},
 doi = {10.1007/978-1-4471-2274-6{\textunderscore }8}
}


@inproceedings{Wang.2008,
 author = {Wang, Ko-Hsin Cindy and Botea, Adi},
 title = {Fast and Memory-Efficient Multi-Agent Pathfinding},
 pages = {380--387},
 booktitle = {ICAPS},
 year = {2008}
}


@article{Wang.2011,
 author = {Wang, Ko-Hsin Cindy and Botea, Adi},
 year = {2011},
 title = {MAPP: a scalable multi-agent path planning algorithm with tractability and completeness guarantees},
 pages = {55--90},
 number = {42},
 journal = {Journal of Artificial Intelligence Research}
}


@patent{Watt.2011,
 author = {Watt, W. J. and Bragg, T. and Stubbs, A. and Verminski, M. D. and Dugan, J. P.},
 year = {2011},
 title = {System and Method for Unloading Items},
 url = {https://www.google.com/patents/US20110103924},
 number = {US20110103924 A1}
}


@misc{Wulfraat.2012b,
 author = {Wulfraat, Marc},
 date = {2012},
 title = {Swisslog Autostore: An In-Depth Review of Automated Split Case Picking Technology for DistributionCenters},
 institution = {{MWPVL International}}
}


@incollection{Wurman.1996,
 author = {Wurman, Peter R. and Wellman, Michael P.},
 title = {Optimal factory scheduling using stochastic dominance A},
 pages = {554--563},
 publisher = {{Morgan Kaufmann Publishers Inc}},
 isbn = {1-55860-412-X},
 booktitle = {Proceedings of the Twelfth international conference on Uncertainty in artificial intelligence},
 year = {1996},
 address = {Portland, OR}
}


@article{Wurman.2008,
 author = {Wurman, Peter R. and D'Andrea, Raffaello and Mountz, Mick},
 DOI = {10.1609/aimag.v29i1.2082},
 title = {Coordinating hundreds of cooperative, autonomous vehicles in warehouses},
 volume = {29},
 year = {2008},
 issn = {0738-4602},
 journal = {AI Magazine}
}


@article{YetkinEkren.2016,
 author = {{Yetkin Ekren}, Banu},
 year = {2016},
 title = {Graph-based solution for performance evaluation of shuttle-based storage and retrieval system},
 pages = {6516--6526},
 volume = {55},
 number = {21},
 issn = {0020-7543},
 journal = {International Journal of Production Research},
 doi = {\url{10.1080/00207543.2016.1203076}}
}


@inproceedings{YiGuo.2002,
 author = {{Yi Guo} and Parker, L. E.},
 title = {A distributed and optimal motion planning approach for multiple mobile robots},
 pages = {2612--2619},
 booktitle = {2002 IEEE International Conference on Robotics and Automation},
 year = {2002},
 doi = {10.1109/ROBOT.2002.1013625}
}


@article{Yu.2009,
 author = {Yu, Mengfei and de Koster, Ren{\'e}},
 year = {2009},
 title = {The impact of order batching and picking area zoning on order picking system performance},
 pages = {480--490},
 volume = {198},
 number = {2},
 issn = {03772217},
 journal = {European Journal of Operational Research},
 doi = {10.1016/j.ejor.2008.09.011}
}


@article{Yuan.2016,
 author = {Yuan, Ruiping and Dong, Tingting and Li, Juntao},
 year = {2016},
 title = {Research on the Collision-Free Path Planning of Multi-AGVs System Based on Improved A* Algorithm},
 pages = {442--449},
 volume = {06},
 number = {06},
 issn = {2160-8830},
 journal = {American Journal of Operations Research},
 doi = {10.4236/ajor.2016.66041}
}


@article{Yuan.2017,
 author = {Yuan, Zhe and Gong, Yeming Yale},
 year = {2017},
 title = {Bot-In-Time Delivery for Robotic Mobile Fulfillment Systems},
 pages = {83--93},
 volume = {64},
 number = {1},
 issn = {0018-9391},
 journal = {IEEE Transactions on Engineering Management},
 doi = {10.1109/TEM.2016.2634540}
}


@article{Zhou.2014,
 author = {Zhou, Luowei and Shi, Yuanyuan and Wang, Jiangliu and Yang, Pei},
 year = {2014},
 title = {A Balanced Heuristic Mechanism for Multirobot Task Allocation of Intelligent Warehouses},
 url = {http://dx.doi.org/10.1155/2014/380480},
 pages = {10},
 volume = {2014},
 journal = {Mathematical Problems in Engineering},
 doi = {10.1155/2014/380480}
}


@article{RawSim.1,
 author = {Merschformann, Marius and Xie, Lin and Li, Hanyi},
 year = {2018},
 month = {08},
 title = {{RAWSim-O}: A Simulation Framework for Robotic Mobile Fulfillment Systems},
 journal = {Logistics Research},
 volume = {11:8}
}

@misc{RawSimDecisionRules,
  author    = {Marius Merschformann and
               Tim Lamballais and
               Ren{\'{e}} de Koster and
               Leena Suhl},
  title     = {Decision Rules for Robotic Mobile Fulfillment Systems},
  url = {https://arxiv.org/pdf/1801.06703.pdf},
  year      = {2018}
}

@article{InventoryAllocation,
author = {Lamballais, Tim and Roy, Debjit and de Koster, M.B.M. René},
year = {2017},
month = {01},
pages = {},
title = {Inventory Allocation in Robotic Mobile Fulfillment Systems},
doi = {10.2139/ssrn.2900940}
}

@misc{Wulfraat.2012,
 author = {Wulfraat, Marc},
 date = {2012},
 year = {2012},
 url = {http://www.mwpvl.com/html/kiva_systems.html},
 title = {Is {K}iva {S}ystems a Good Fit for Your Distribution Center? {A}n Unbiased Distribution Consultant Evaluation.},
 institution = {{MWPVL International}}
}


@article{Boysen.2017,
	title={Parts-to-picker based order processing in a rack-moving mobile robots environment},
	author={Boysen, Nils and Briskorn, Dirk and Emde, Simon},
	journal={European Journal of Operational Research},
	volume={262},
	number={2},
	pages={550--562},
	year={2017},
	doi={10.1016/j.ejor.2017.03.053},
	publisher={Elsevier}
}
@misc{Mittelmann.2018,
 author = {Mittelmann, Hans Detlef},
 date = {2018},
 year = {2018},
 url = {http://plato.asu.edu/ftp/milpc.html},
 title = {Mixed Integer Linear Programming Benchmark},
 institution = {School of Math & Stats, Arizona State University}
}


@misc{Xie.2018,
   author = {{Xie}, L. and {Li}, H. and {Thieme}, N.},
    title = {From Simulation to Real-World Robotic Mobile Fulfillment Systems},
    year = 2019,
    journal = {Logistics Research},
    doi = {DOI_10.23773/2019_9},
    volume = {12:9}
}
}

@article{Armstron.1979,
	title={Optimal batching in a semi-automated order picking system},
	author={Armstrong, Ronald D and Cook, Wade D and Saipe, Alan L},
	journal={Journal of the Operational Research Society},
	volume={30},
	number={8},
	pages={711--720},
	year={1979},
	publisher={Taylor \& Francis}
}

@misc{overview.old,
 URL = {https://www2.isye.gatech.edu/~mgoetsch/cali/Logistics\%20Tutorial/order/article.htm},
 year = {1991},
 date = {1991},
 author = {Kyung Il-Choe and Gunter Sharp},
 title = {Small Parts Order Picking: Design and Operation},
}

@article{sortingsystems,
author = { Mardi L. Russell  and  Russell D. Meller },
title = {Cost and Throughput Modeling of Manual and Automated Order Fulfillment Systems},
journal = {IIE Transactions},
volume = {35 (2003)},
publisher = {Taylor & Francis},
doi = {10.1080/07408170304358},
}

@misc{pathplanning,
  author    = {Marius Merschformann and
               Lin Xie and
               Daniel Erdmann},
  title     = {Path planning for Robotic Mobile Fulfillment Systems},
  year      = {2017},
  url = {https://arxiv.org/pdf/1706.09347.pdf}
  }

@book{Tompkins.2010,
	author = {Tompkins, James A.},
	year = {2010},
	title = {Facilities planning},
	edition = {4th ed.},
	publisher = {{John Wiley {\&} Sons}},
	isbn = {0470444045}
}

@book{bartholdi.2017,
  title={Warehouse \& Distribution Science: Release 0.98},
  author={Bartholdi, J.J. and Hackman, S.T.},
  url={https://www.warehouse-science.com/book/},
  publisher={Supply Chain and Logistics Institute},
  year={2017}
}


@Comment{jabref-meta: databaseType:biblatex;}

@article{de2012determining,
	title={Determining the number of zones in a pick-and-sort order picking system},
	author={De Koster, Ren{\'e} BM and Le-Duc, Tho and Zaerpour, Nima},
	journal={International Journal of Production Research},
	volume={50},
	number={3},
	pages={757--771},
	year={2012},
	doi={10.1080/00207543.2010.543941},
	publisher={Taylor \& Francis}
}

@misc{banker2016robots,
	title={Robots in the warehouse: It’s not just {A}mazon},
	author={Banker, S},
	url={http://www.forbes.com},
	year={2016}
}

@misc{patent-wurman-brunner-barbehenn:2013,
	title={Method and system for fulfilling requests in an inventory system},
	author={Wurman, Peter R and Brunner, Daniel T and Barbehenn, Michael T},
	year={2013},
	publisher={Google Patents},
	note={US Patent 8,483,869}
}

@article{bozer2018simulation,
	author = {Yavuz A. Bozer and Francisco J. Aldarondo},
	title = {A simulation-based comparison of two goods-to-person order picking systems in an online retail setting},
	journal = {International Journal of Production Research},
	volume = {56},
	number = {11},
	pages = {3838-3858},
	year  = {2018},
	publisher = {Taylor & Francis},
	doi = {10.1080/00207543.2018.1424364}
}

@article{onal2017modelling,
	title={Modelling and performance evaluation of explosive storage policies in internet fulfilment warehouses},
	author={Onal, Sevilay and Zhang, Jingran and Das, Sanchoy},
	journal={International Journal of Production Research},
	volume={55},
	number={20},
	pages={5902--5915},
	year={2017},
	publisher={Taylor \& Francis}
}

@article{de2007design,
	title={Design and control of warehouse order picking: A literature review},
	author={De Koster, Ren{\'e} and Le-Duc, Tho and Roodbergen, Kees Jan},
	journal={European {J}ournal of {O}perational {R}esearch},
	volume={182},
	number={2},
	pages={481--501},
	year={2007},
	doi={10.1016/j.ejor.2006.07.009},
	publisher={Elsevier}
}

@misc{krenzler2018deterministic,
	title={Deterministic Pod Repositioning Problem in Robotic Mobile Fulfillment Systems},
	author={Krenzler, Ruslan and Xie, Lin and Li, Hanyi},
	url = {https://arxiv.org/pdf/1810.05514.pdf},
	year={2018}
}

@misc{Cohen.20170608,
	author = {Cohen, Liron and Wagner, Glenn and Kumar, T. K. Satish and Choset, Howie and Koenig, Sven},
	year = {2017},
	title = {Rapid Randomized Restarts for Multi-Agent Path Finding Solvers},
	url = {http://arxiv.org/pdf/1706.02794}
}
@misc{website:packing,
	author = "Toister, Jeff",
	title = "An Inside Look at {A}mazon's Fulfillment Center Operations",
	month = "April",
	year = "2017",
	url = "https://www.toistersolutions.com/blog/2017/4/10/an-inside-look-at-amazons-fulfillment-center-operations"
}
@misc{flipse2011altering,
	title={Altering and improving {K}iva},
	author={Flipse, Marcel},
	year={2011},
	note={Working Paper, Vrije Universiteit Amsterdam}
}
@article{boysen2019warehousing,
	title={Warehousing in the e-commerce era: A survey},
	author={Boysen, Nils and de Koster, Ren{\'e} and Weidinger, Felix},
	journal={European Journal of Operational Research},
	volume={277},
	number={2},
	pages={396--411},
	year={2019},
	doi={10.1016/j.ejor.2018.08.023},
	publisher={Elsevier}
}
@article{zhang2019building,
	title={A Building-Block-Based Genetic Algorithm for Solving the Robots Allocation Problem in a Robotic Mobile Fulfilment System},
	author={Zhang, Jingtian and Yang, Fuxing and Weng, Xun},
	journal={Mathematical Problems in Engineering},
	volume={2019},
	year={2019},
	publisher={Hindawi}
}

@article{hanson2018performance,
	title={Performance Characteristics of Robotic Mobile Fulfilment Systems in Order Picking Applications},
	author={Hanson, Robin and Medbo, Lars and Johansson, Mats I},
	journal={IFAC-PapersOnLine},
	volume={51},
	number={11},
	pages={1493--1498},
	year={2018},
	publisher={Elsevier}
}
@article{yuan2017bot,
	title={Bot-in-time delivery for robotic mobile fulfillment systems},
	author={Yuan, Zhe and Gong, Yeming Yale},
	journal={IEEE Transactions on Engineering Management},
	volume={64},
	number={1},
	pages={83--93},
	year={2017},
	publisher={IEEE}
}
@article{zou2017assignment,
	title={Assignment rules in robotic mobile fulfilment systems for online retailers},
	author={Zou, Bipan and Gong, Yeming and Xu, Xianhao and Yuan, Zhe},
	journal={International Journal of Production Research},
	volume={55},
	number={20},
	pages={6175--6192},
	year={2017},
	publisher={Taylor \& Francis}
}
@article{lee2019robotics,
	title={Robotics in order picking: {E}valuating warehouse layouts for pick, place, and transport vehicle routing systems},
	author={Lee, Hung-Yu and Murray, Chase C},
	journal={International Journal of Production Research},
	volume={57},
	number={18},
	pages={5821--5841},
	year={2019},
	doi={10.1080/00207543.2018.1552031},
	publisher={Taylor \& Francis}
}
@article{cheng2015using,
	title={Using a hybrid approach based on the particle swarm optimization and ant colony optimization to solve a joint order batching and picker routing problem},
	author={Cheng, Chen-Yang and Chen, Yin-Yann and Chen, Tzu-Li and Yoo, John Jung-Woon},
	journal={International Journal of Production Economics},
	volume={170},
	pages={805--814},
	year={2015},
	doi={10.1016/j.ijpe.2015.03.021},
	publisher={Elsevier}
}
@article{ene2012storage,
	title={Storage location assignment and order picking optimization in the automotive industry},
	author={Ene, Seval and {\"O}zt{\"u}rk, Nursel},
	journal={The International Journal of Advanced Manufacturing Technology},
	volume={60},
	number={5-8},
	pages={787--797},
	year={2012},
	doi={10.1007/s00170-011-3593-y},
	publisher={Springer}
}
@article{kulak2012joint,
	title={Joint order batching and picker routing in single and multiple-cross-aisle warehouses using cluster-based tabu search algorithms},
	author={Kulak, Osman and Sahin, Yusuf and Taner, Mustafa Egemen},
	journal={Flexible Services and Manufacturing Journal},
	volume={24},
	number={1},
	pages={52--80},
	year={2012},
	doi={10.1007/s10696-011-9101-8},
	publisher={Springer}
}
@article{li2017joint,
	title={Joint optimisation of order batching and picker routing in the online retailer’s warehouse in {China}},
	author={Li, Jianbin and Huang, Rihuan and Dai, James B},
	journal={International Journal of Production Research},
	volume={55},
	number={2},
	pages={447--461},
	year={2017},
	doi={10.1080/00207543.2016.1187313},
	publisher={Taylor \& Francis}
}
@article{matusiak2014fast,
	title={A fast simulated annealing method for batching precedence-constrained customer orders in a warehouse},
	author={Matusiak, Marek and de Koster, Ren{\'e} and Kroon, Leo and Saarinen, Jari},
	journal={European Journal of Operational Research},
	volume={236},
	number={3},
	pages={968--977},
	year={2014},
	doi={10.1016/j.ejor.2013.06.001},
	publisher={Elsevier}
}
@article{tsai2008using,
	title={Using a multiple-{GA} method to solve the batch picking problem: {C}onsidering travel distance and order due time},
	author={Tsai, C-Y and Liou, James JH and Huang, T-M},
	journal={International Journal of Production Research},
	volume={46},
	number={22},
	pages={6533--6555},
	year={2008},
	doi={10.1080/00207540701441947},
	publisher={Taylor \& Francis}
}
@article{valle2017optimally,
	title={Optimally solving the joint order batching and picker routing problem},
	author={Valle, Cristiano Arbex and Beasley, John E and da Cunha, Alexandre Salles},
	journal={European Journal of Operational Research},
	volume={262},
	number={3},
	pages={817--834},
	year={2017},
	doi={10.1016/j.ejor.2017.03.069},
	publisher={Elsevier}
}
@article{won2005joint,
	title={Joint order batching and order picking in warehouse operations},
	author={Won, J and Olafsson, S},
	journal={International Journal of Production Research},
	volume={43},
	number={7},
	pages={1427--1442},
	year={2005},
	doi={10.1080/00207540410001733896},
	publisher={Taylor \& Francis}
}
@article{lin2016joint,
	title={Joint order batching and picker {Manhattan} routing problem},
	author={Lin, Chun-Cheng and Kang, Jia-Rong and Hou, Chung-Chih and Cheng, Chen-Yang},
	journal={Computers \& Industrial Engineering},
	volume={95},
	pages={164--174},
	year={2016},
	doi={10.1016/j.cie.2016.03.009},
	publisher={Elsevier}
}
@article{van2019formulating,
	title={Formulating and solving the integrated batching, routing, and picker scheduling problem in a real-life spare parts warehouse},
	author={Van Gils, Teun and Caris, An and Ramaekers, Katrien and Braekers, Kris},
	journal={European Journal of Operational Research},
	volume={277},
	number={3},
	pages={814--830},
	year={2019},
	doi={10.1016/j.ejor.2019.03.012},
	publisher={Elsevier}
}
@article{chen2015efficient,
	title={An efficient hybrid algorithm for integrated order batching, sequencing and routing problem},
	author={Chen, Tzu-Li and Cheng, Chen-Yang and Chen, Yin-Yann and Chan, Li-Kai},
	journal={International Journal of Production Economics},
	volume={159},
	pages={158--167},
	year={2015},
	doi={10.1016/j.ijpe.2014.09.029},
	publisher={Elsevier}
}
@article{scholz2017order,
	title={Order picking with multiple pickers and due dates: {S}imultaneous solution of order batching, batch assignment and sequencing, and picker routing problems},
	author={Scholz, Andr{\'e} and Schubert, Daniel and W{\"a}scher, Gerhard},
	journal={European Journal of Operational Research},
	volume={263},
	number={2},
	pages={461--478},
	year={2017},
	doi={10.1016/j.ejor.2017.04.038},
	publisher={Elsevier}
}
@article{weidinger2019picker,
	title={Picker routing in the mixed-shelves warehouses of e-commerce retailers},
	author={Weidinger, Felix and Boysen, Nils and Schneider, Michael},
	journal={European Journal of Operational Research},
	volume={274},
	number={2},
	pages={501--515},
	year={2019},
	doi={10.1016/j.ejor.2018.10.021},
	publisher={Elsevier}
}
@article{van2018designing,
	title={Designing efficient order picking systems by combining planning problems: State-of-the-art classification and review},
	author={Van Gils, Teun and Ramaekers, Katrien and Caris, An and De Koster, Ren{\'e} BM},
	journal={European Journal of Operational Research},
	volume={267},
	number={1},
	pages={1--15},
	year={2018},
	doi={10.1016/j.ejor.2017.09.002},
	publisher={Elsevier}
}
@article{baldacci2004exact,
	title={An exact algorithm for the capacitated vehicle routing problem based on a two-commodity network flow formulation},
	author={Baldacci, Roberto and Hadjiconstantinou, Eleni and Mingozzi, Aristide},
	journal={Operations Research},
	volume={52},
	number={5},
	pages={723--738},
	year={2004},
	doi={10.1287/opre.1040.0111},
	publisher={INFORMS}
}
@article{ramos2019multi,
	title={Multi-depot vehicle routing problem: {A} comparative study of alternative formulations},
	author={Ramos, T{\^a}nia Rodrigues Pereira and Gomes, Maria Isabel and P{\'o}voa, Ana Paula Barbosa},
	journal={International Journal of Logistics Research and Applications},
	volume={23},
	number={2},
	pages={103--120},
	year={2020},
	doi={10.1080/13675567.2019.1630374},
	publisher={Taylor \& Francis}
}
@article{finke1984two,
	title={A two-commodity network flow approach to the traveling salesman problem},
	author={Finke, Gerd},
	journal={Congressus Numerantium},
	volume={41},
	pages={167--178},
	year={1984}
}
@article{xie2019efficient,
	title={Introducing split orders and optimizing operational policies in robotic mobile fulfillment systems},
	author={Xie, Lin and Thieme, Nils and Krenzler, Ruslan and Li, Hanyi},
	journal={European Journal of Operational Research},
	doi = {https://doi.org/10.1016/j.ejor.2020.05.032},
	year={2020}
}
@article{dror1989savings,
	title={Savings by split delivery routing},
	author={Dror, Moshe and Trudeau, Pierre},
	journal={Transportation Science},
	volume={23},
	number={2},
	pages={141--145},
	year={1989},
	publisher={INFORMS}
}
@article{dror1990split,
	title={Split delivery routing},
	author={Dror, Moshe and Trudeau, Pierre},
	journal={Naval Research Logistics (NRL)},
	volume={37},
	number={3},
	pages={383--402},
	year={1990},
	publisher={Wiley Online Library}
}
@article{azadeh2019robotized,
	title={Robotized and automated warehouse systems: Review and recent developments},
	author={Azadeh, Kaveh and De Koster, Ren{\'e} and Roy, Debjit},
	journal={Transportation Science},
	volume={53},
	number={4},
	pages={917--945},
	year={2019},
	doi={10.1287/trsc.2018.0873},
	publisher={INFORMS}
}
@article{daniels1998model,
	title={A model for warehouse order picking},
	author={Daniels, Richard L and Rummel, Jeffrey L and Schantz, Robert},
	journal={European Journal of Operational Research},
	volume={105},
	number={1},
	pages={1--17},
	year={1998},
	doi={10.1016/S0377-2217(97)00043-X},
	publisher={Elsevier}
}
@techreport{loffler2018picker,
	title={Picker routing in AGV-assisted order picking systems},
	author={L{\"o}ffler, M and Boysen, N and Schneider, M},
	year={2018},
	institution={Working Paper, DPO-01/2018, Deutsche Post Chair-Optimization of Distribution Networks, RWTH Aachen University}
}
@article{weidinger2018picker,
	title={Picker routing in rectangular mixed shelves warehouses},
	author={Weidinger, Felix},
	journal={Computers \& Operations Research},
	volume={95},
	pages={139--150},
	year={2018},
	doi={10.1016/j.cor.2018.03.012},
	publisher={Elsevier}
}
@article{montoya2015literature,
	title={A literature review on the vehicle routing problem with multiple depots},
	author={Montoya-Torres, Jairo R and Franco, Juli{\'a}n L{\'o}pez and Isaza, Santiago Nieto and Jim{\'e}nez, Heriberto Felizzola and Herazo-Padilla, Nilson},
	journal={Computers \& Industrial Engineering},
	volume={79},
	pages={115--129},
	year={2015},
	doi={10.1016/j.cie.2014.10.029},
	publisher={Elsevier}
}
@article{nowak2008pickup,
	title={Pickup and delivery with split loads},
	author={Nowak, Maciek and Ergun, {\"O}zlem and White III, Chelsea C},
	journal={Transportation Science},
	volume={42},
	number={1},
	pages={32--43},
	year={2008},
	publisher={INFORMS}
}
@article{nowak2009empirical,
	title={An empirical study on the benefit of split loads with the pickup and delivery problem},
	author={Nowak, Maciek and Ergun, Ozlem and White III, Chelsea C},
	journal={European Journal of Operational Research},
	volume={198},
	number={3},
	pages={734--740},
	year={2009},
	publisher={Elsevier}
}
@misc{Wulfraat.2016,
	author = {Wulfraat, Marc},
	month = {May},
	year = {2016},
	url = {https://mwpvl.com/html/locus_robotics_-_independent_consultant_review.html},
	title = {{L}ocus {R}obotics: {A}n Independent Consultant Review of Autonomous Robots},
	institution = {{MWPVL International}}
}
@article{weidinger2018scattered,
	title={Scattered storage: How to distribute stock keeping units all around a mixed-shelves warehouse},
	author={Weidinger, Felix and Boysen, Nils},
	journal={Transportation Science},
	volume={52},
	number={6},
	pages={1412--1427},
	year={2018},
	doi={10.1287/trsc.2017.0779},
	publisher={INFORMS}
}
@article{baldacci2007recent,
	title={Recent advances in vehicle routing exact algorithms},
	author={Baldacci, Roberto and Toth, Paolo and Vigo, Daniele},
	journal={4OR},
	volume={5},
	number={4},
	pages={269--298},
	year={2007},
	doi={10.1007/s10288-007-0063-3},
	publisher={Springer}
}
@InProceedings{networkX,
 	author =       {Aric A. Hagberg and Daniel A. Schult and Pieter J. Swart},
	title =        {Exploring Network Structure, Dynamics, and Function using {NetworkX}},
	booktitle =   {Proceedings of the 7th Python in Science Conference},
	pages =     {11--15},
	address = {Pasadena, CA, USA},
	year =      {2008},
	editor =    {Ga\"el Varoquaux and Travis Vaught and Jarrod Millman},
}
@misc{fabric.2020,
	author = {Fabric},
	date = {2020},
	year = {2020},
	url = {https://getfabric.com/the-impact-of-covid-19-on-online-grocery/},
	title = {{The impact of Covid-19 on online grocery: Why the coronavirus pandemic in 2020 will change the grocery industry forever in the United States}},
}

@book{garey1979computers,
	title={Computers and intractability: {A} guide to the theory of {NP}-completeness},
	author={Garey, Michael R and Johnson, David S},
	volume={174},
	year={1979},
	publisher={Freeman}
}
@article{letchford2013compact,
	title={Compact formulations of the {S}teiner traveling salesman problem and related problems},
	author={Letchford, Adam N and Nasiri, Saeideh D and Theis, Dirk Oliver},
	journal={European Journal of Operational Research},
	volume={228},
	number={1},
	pages={83--92},
	year={2013},
	doi={10.1016/j.ejor.2013.01.044},
	publisher={Elsevier}
}
@book{gendreau2010handbook,
	title={Handbook of metaheuristics},
	author={Gendreau, Michel and Potvin, Jean-Yves (Eds.)},
	volume={3},
	year={2010},
	doi={10.1007/978-3-319-91086-4},
	publisher={Springer}
}
@article{kytojoki2007efficient,
	title={An efficient variable neighborhood search heuristic for very large scale vehicle routing problems},
	author={Kyt{\"o}joki, Jari and Nuortio, Teemu and Br{\"a}ysy, Olli and Gendreau, Michel},
	journal={Computers \& Operations Research},
	volume={34},
	number={9},
	pages={2743--2757},
	year={2007},
	doi={10.1016/j.cor.2005.10.010},
	publisher={Elsevier}
}
@article{briant2020efficient,
	title={An efficient and general approach for the joint order batching and picker routing problem},
	author={Briant, Olivier and Cambazard, Hadrien and Cattaruzza, Diego and Catusse, Nicolas and Ladier, Anne-Laure and Ogier, Maxime},
	journal={European Journal of Operational Research},
	volume={285},
	number={2},
	pages={497--512},
	year={2020},
	doi={10.1016/j.ejor.2020.01.059},
	publisher={Elsevier}
}
@article{kubler2020new,
	title={A new iterative method for solving the joint dynamic storage location assignment, order batching and picker routing problem in manual picker-to-parts warehouses},
	author={K{\"u}bler, Patrick and Glock, Christoph H and Bauernhansl, Thomas},
	journal={Computers \& Industrial Engineering},
	volume={147},
	pages={106645},
	year={2020},
	doi={10.1016/j.cie.2020.106645},
	publisher={Elsevier}
}
@article{mladenovic1997variable,
	title={Variable neighborhood search},
	author={Mladenovi{\'c}, Nenad and Hansen, Pierre},
	journal={Computers \& Operations Research},
	volume={24},
	number={11},
	pages={1097--1100},
	year={1997},
	doi={10.1016/S0305-0548(97)00031-2},
	publisher={Elsevier}
}
@article{giosa2002new,
	title={New assignment algorithms for the multi-depot vehicle routing problem},
	author={Giosa, ID and Tansini, IL and Viera, IO},
	journal={Journal of the Operational Research Society},
	volume={53},
	number={9},
	pages={977--984},
	year={2002},
	doi={10.1057/palgrave.jors.2601426},
	publisher={Taylor \& Francis}
}

@inProceedings{Alvim99localsearch,
	author = {Adriana Alvim and Fred S. Glover and Celso C. Ribeiro and Dario J. Aloise},
	title = {Local Search For The Bin Packing Problem},
	booktitle ={Extended Abstracts of the 3rd Metaheuristics International Conference},
	pages={7--12},
	year = {1999},
	publisher={CiteSeer}
}

@book{karmarkar1982differencing,
  title={The differencing method of set partitioning},
  author={Karmarkar, Narendra and Karp, Richard M},
  year={1982},
  publisher={Computer Science Division (EECS), University of California}
}

@book{gendreau2010handbook,
  title={Handbook of metaheuristics},
  author={Gendreau, Michel and Potvin, Jean-Yves and others},
  volume={2},
  year={2010},
  publisher={Springer}
}
